Perceive With Confidence: Statistical Safety Assurances for Navigation with Learning-Based Perception

Rapid advances in perception have enabled large pre-trained models to be used out of the box for transforming high-dimensional, noisy, and partial observations of the world into rich occupancy representations. However, the reliability of these models and consequently their safe integration onto robots remains unknown when deployed in environments unseen during training. To provide safety guarantees, we rigorously quantify the uncertainty of pre-trained perception systems for object detection and scene completion via a novel calibration technique based on conformal prediction. Crucially, this procedure guarantees robustness to distribution shifts in states when perception outputs are used in conjunction with a planner. As a result, the calibrated perception system can be used in combination with any safe planner to provide an end-to-end statistical assurance on safety in unseen environments. We evaluate the resulting approach, Perceive with Confidence (PwC), in simulation and on hardware where a quadruped robot navigates through previously unseen indoor, static environments. These experiments validate the safety assurances for obstacle avoidance provided by PwC. In simulation, our method reduces obstacle misdetection by $70\%$ compared to uncalibrated perception models. While misdetections lead to collisions for baseline methods, our approach consistently achieves $100\%$ safety. We further demonstrate reducing the conservatism of our method without sacrificing safety, achieving a $46\%$ increase in success rates in challenging environments while maintaining $100\%$ safety. In hardware experiments, our method improves empirical safety by $40\%$ over baselines and reduces obstacle misdetection by $93.3\%$. The safety gap widens to $46.7\%$ when navigation speed increases, highlighting our approach's robustness under more demanding conditions.

==> sections/drone.tex <==

\jimmy{
\subsection{Validation on Drone Navigation.}
\label{sec:drone}
We further evaluate the modularity of our proposed approach by integrating it with an in-house quadrotor platform for hardware testing. The base system of our quadrotor was originally developed by the Robotics and Perception Group at the University of Zurich, as described in their paper on \textit{Agilicious} \citep{foehn2022agilicious}. The \textit{Agilicious} framework comprises of a standard racing drone (flight controller, ESC board, motors, etc.) equipped with a 16GB Jetson Orin NX compute unit serial-bridged to the drone’s flight controller (running Betaflight software) via UART communication. In addition, \textit{Agilicious} integrates a Realsense T265 visual-inertial odometry camera and a VICON motion capture ROS listener node for two different means of state estimation (onboard and ground truth, respectively). Researchers in the Intelligent Robot Motion Lab extended \textit{Agilicious} by implementing a depth-based motion planning pipeline on top of the base framework. This pipeline incorporates a bridge script that transports depth point clouds captured via an onboard Realsense D435 stereo-depth camera (with a field of view of $87^\circ$, and a visibility range of [0.3,3]m) to a running planner. The planner then processes the point cloud, generates a trajectory, and sends waypoint commands back over a ROS network to be handled by the \textit{Agilicious} pilot. We perform an initial round of tests utilizing the concurrent planning framework on the quadrotor at speeds of 0.5 to 1 m/s, navigating in varying configurations of 3-5 chairs inside a 4m x 8m room. As an early-stage proof of concept, this demonstrates that our approach can be integrated with different hardware platforms, opening future venues to expand the work presented in this paper.}



 
 
 This approach is especially strong for hard detection scenarios such as the one illustrated in Fig. \ref{fig:chair}. In the first trial (Fig. \ref{fig:chair_easy}), both approaches detect the chair and navigate around it. However, when the chair is turned to directly face the robot (Fig. \ref{fig:chair_hard}), chair features become harder to detect. The baseline entirely misdetects this chair and crashes into it while our approach is able to inflate the bounding box detections that do appear (despite them being poor) and then shrink the free space estimate quickly with the nondeterministic filter.


reference video\\
create figs that show nice qual. results and discuss:\\
maybe occluded chair, the tight space one, and hard to detect chair (the one facing directly forward as a rectangle) \\
and one scenario showing evolution of free space updates and plans (maybe hard to detect one)\\
discuss pwc crash cases

\vspace{2mm}

\begin{tabular}{ p{1.5cm} p{1.5cm} p{1.5cm} p{1cm} p{0.5cm} p{1cm}}
 \hline
\textbf{Method} & \textbf{Collisions} &\textbf{Misdetections} & \textbf{Path length} & \textbf{Succ.} & \textbf{Dist. to goal}\\
 \hline
 PwC & $0$    & $0 $ & $0$ \\
 \hline
 CP = 0.02 \citep{} & $0$    & $0 $ & $0$ \\
 \hline

 

\end{tabular}

\end{itemize}
